Generalized and Scalable Optimal Sparse Decision Trees

Decision tree optimization is notoriously difficult from a computational perspective but essential for the field of interpretable machine learning. Despite efforts over the past 40 years, only recently have optimization breakthroughs been made that have allowed practical algorithms to find optimal decision trees. These new techniques have the potential to trigger a paradigm shift where it is possible to construct sparse decision trees to efficiently optimize a variety of objective functions without relying on greedy splitting and pruning heuristics that often lead to suboptimal solutions. The contribution in this work is to provide a general framework for decision tree optimization that addresses the two significant open problems in the area: treatment of imbalanced data and fully optimizing over continuous variables. We present techniques that produce optimal decision trees over a variety of objectives including F-score, AUC, and partial area under the ROC convex hull. We also introduce a scalable algorithm that produces provably optimal results in the presence of continuous variables and speeds up decision tree construction by several orders of magnitude relative to the state-of-the art.

==> mainOld.tex <==
% \documentclass{article}
% \usepackage[utf8]{inputenc}

% \title{Generalized Scalable Optimal Sparse Decision Trees}
% \author{Jimmy and Chudi as co-first authors, Margo and Cynthia, not sure what order}
% \date{September 2019}

% \begin{document}
% \maketitle
% \begin{abstract}
% Decision tree optimization is notoriously difficult from a computational perspective, but essential for the field of interpretable machine learning. Despite efforts over the past 40 years, only recently have optimization breakthroughs been made that have allowed practical algorithms to find \textit{optimal} decision trees. These new techniques have the potential to trigger a paradigm shift, where, ideally, sparse decision trees can be constructed to efficiently optimize a variety of objective functions, without relying on greedy splitting and pruning heuristics that often lead to suboptimal solutions. The contribution in this work is to enable this paradigm shift by providing a general framework for decision tree optimization, that includes a wide variety of objectives such as AUC, partial AUC, ???. Our framework includes a scalable algorithm that speeds up decision tree code by several order of magnitude from the previous state-of-the art, through a new dynamic-programming-with-bounds (DPB) algorithm. This new algorithm handles a known -- but previously unsolved -- challenge in decision tree optimization, namely how to handle mixed continuous and discrete variables in reasonable run-times for practical problems.
% \end{abstract}
% \section{Introduction}
% Decision tree learning has served as a foundation for interpretable artificial intelligence and machine learning for several decades, with roots starting from the expert systems literature from when computers were first introduced in the 1940's and 50's. At the time, people wanted to design computers that could mimic the if-then reasoning of a human expert \citep{???}. Since that time, different types of approaches have been used for decision tree learning. The major approach since the 1980's has been decision tree induction, where heuristic splitting and pruning procedures grow a tree from the top down and prune it back afterwards \citep{CART,C4.5}. The problem with these methods is that they tend to produce suboptimal trees, and there is no way to know how suboptimal the solution is. This leaves a gap between the performance that \textit{might} be obtained by a decision tree, and the performance that one actually attains, with no way to check on (or remedy) the size of this gap. This gap can be large: the CART algorithm \citep{CART}, for example, often produces trivial trees--that predict all one class--on imbalanced problems, even if one attempts to vary the parameters that control its performance on imbalanced data \citep{??}.

% Greedy splitting and pruning for decision tree induction have dominated for decades, despite serious attempts to change the paradigm away from using heuristics to optimize decision trees. These attempts aimed to optimize the full set of decision tree nodes to maximize prediction accuracy, subject to constraints or regularization on the tree's size. Full decision tree optimization is NP-hard, with no polynomial-time approximation \citep{??}, which has led to practical challenges in proving optimality, or bounding the optimality gap, in reasonable amounts of time, even for small datasets. 
% %As a result, heuristics are still the state-of-the art. 
% Mathematical programming solvers started to be used for this in the 1990's \citep{BennettBlue}, continuing to the present \cite{Others??, ErtekinRu??}, but these generic solvers tend to be slow to converge. To our knowledge, the most promising approach to this problem with mathematical solvers is the BinOct algorithm \citep{BinOct}, which simplifies the problem to that of finding \textit{complete} optimal decision trees of a fixed depth. Two problems with this approach are that (i) even if a smaller tree is equally accurate, BinOct fills in the remaining leaves to form a (unnecessarily large) complete tree, and (ii) BinOct is very slow to prove optimality when handling splits on continuous variables, owing to its use of generic solvers.

% Significant breakthroughs in 2018-2019 have led to hope of change for decision tree optimization. 
% A completely different approach--using neither all-purpose optimization solvers nor heuristics--was introduced in the CORELS algorithm \citep{AngelinoEtAl17,AngelinoEtAl19}, which is actually an associative classification method. Like traditional decision trees, associative classifiers are based on if-then rules, but they can include multiple conditions within each split (if $a$ AND $b$, then predict $Y$=1, else if ...), permitting for more flexible models for a given depth. Like decision trees, associative classifiers have also traditionally been built using greedy methods \citep[e.g.,][]{???} or mathematical programming solvers \citep[e.g.,][]{ErtekinRu}. CORELS breaks apart from the previous literature on either optimal decision trees or associative classification in that it is a custom branch-and-bound method, with  custom bounding theorems, its own bit-vector library, and it leverages computational reuse. CORELS is able to solve problems within only a minute that, using any other prior approach, might have taken weeks, or even months or years.

% The CORELS framework was migrated to handle full binary-split decision trees in the Optimal Sparse Decision Tree (ODST) algorithm \cite{HuEtAl}, which preserved CORELS' libraries, computational reuse, and many of its theorems to reduce the size of the search space. However, OSDT solves an exponentially harder problem than that of CORELS' rule list optimization, leading to challenges in scalability. 
% %This leaves two major challenges: 

% The contributions of this work are (1) to massively generalize sparse decision tree optimization to handle a wide variety of objective functions, and (2) to present a new optimization method for decision tree optimization using a new dynamic-programming-with-bounds technique.

% Let us discuss goal (1), which is to consider a wide variety of objective functions. Both CORELS and OSDT were designed to maximize accuracy, regularized by sparsity, and neither are designed to handle other objectives. CORELS has been generalized \citep{FairCORELS,ChenRu19} to handle various interpretability and fairness constraints, but not (as far as we know) to the wide variety of different objectives one might want to handle in practice. Generalization to some of the objectives we consider is straightforward (e.g., imbalanced classification) but non-trivial in cases of optimizing rank statistics (e.g., partial area under the convex hull of the ROC curve), which typically require quadratic computation in the number of observations in the dataset. However, for sparse decision trees, this time is much less than quadratic, owing to the fact that all observations within a leaf of a tree are tied in score, and because there are a sparse number of leaves in the tree. This permits us to rapidly calculate rank statistics, and thus, optimize over them. (Note that we do not use convex proxies for rank statistics, which are problematic in that they can be distant from the rank statistic they aim to approximate \cite{RudinWa18}, we optimize these rank statistics directly on the training set.)

% For goal (2), we designed a 





% \maketitle

% \section{Introduction}

% \end{document}

